Secrecy Energy Efficiency Maximization in RIS-Aided Wireless Networks with Statistical CSI

This work studies the problem of secrecy energy efficiency maximization in multi-user wireless networks aided by reconfigurable intelligent surfaces, in which an eavesdropper overhears the uplink communication. A provably convergent optimization algorithm is proposed which optimizes the user's transmit power, metasurface reflection coefficients, and base station receive filters. The complexity of the proposed method is analyzed and numerical results are provided to show the performance of the proposed optimization method.

==> abbreviations.tex <==
%\renewcommand{\arraystretch}{1.5}
%\newcommand{\spazio}{\rule[-6mm]{0mm}{0mm}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\wt}{\widetilde}
\newcommand{\ov}{\overline}
\newcommand{\LL}{{\cal L}}
\newcommand{\bN}{\mbox{\boldmath $N$}}
\newcommand{\br}{\mbox{\boldmath $r$}}
\newcommand{\bT}{\mbox{\boldmath $T$}}
\newcommand{\bJ}{\mbox{\boldmath $J$}}
\newcommand{\bs}{\mbox{\boldmath $s$}}
\newcommand{\uH}{\underline{H}}
\newcommand{\uh}{\underline{h}}
\newcommand{\bb}{\mbox{\boldmath $b$}}
\newcommand{\bbf}{\mbox{\boldmath $f$}}
\newcommand{\ba}{\mbox{\boldmath $a$}}
\newcommand{\bq}{\mbox{\boldmath $q$}}
\newcommand{\bp}{\mbox{\boldmath $p$}}
\newcommand{\be}{\mbox{\boldmath $e$}}
\newcommand{\bzero}{\mbox{\boldmath $0$}}
\newcommand{\bM}{\mbox{\boldmath $M$}}
\newcommand{\wi}{\widetilde}
\newcommand{\bDelta}{\mbox{\boldmath $\Delta$}}
\newcommand{\wh}{\widehat}
\newcommand{\bA}{\mbox{\boldmath $A$}}
\newcommand{\bP}{\mbox{\boldmath $P$}}
\newcommand{\bC}{\mbox{\boldmath $C$}}
\newcommand{\bX}{\mbox{\boldmath $X$}}
\newcommand{\bh}{\mbox{\boldmath $h$}}
\newcommand{\bH}{\mbox{\boldmath $H$}}
\newcommand{\bK}{\mbox{\boldmath $K$}}
\newcommand{\bk}{\mbox{\boldmath $k$}}
\newcommand{\bc}{\mbox{\boldmath $c$}}
\newcommand{\bS}{\mbox{\boldmath $S$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bZ}{\mbox{\boldmath $Z$}}
\newcommand{\bU}{\mbox{\boldmath $U$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bB}{\mbox{\boldmath $B$}}
\newcommand{\bE}{\mbox{\boldmath $E$}}
\newcommand{\bV}{\mbox{\boldmath $V$}}
\newcommand{\bL}{\mbox{\boldmath $L$}}
\newcommand{\bG}{\mbox{\boldmath $G$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bW}{\mbox{\boldmath $W$}}
\newcommand{\bLambda}{{\bf \Lambda}}
\newcommand{\bpsi}{{\bf \Psi}}
\newcommand{\bPsi}{{\bf \Psi}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
%\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bi}{\mbox{\boldmath $i$}}
\newcommand{\bu}{\mbox{\boldmath $u$}}
\newcommand{\bzeta}{\mbox{\boldmath $\zeta$}}
\newcommand{\bdelta}{\mbox{\boldmath $\delta$}}
\newcommand{\bx}{\mbox{\boldmath $x$}}
\newcommand{\bz}{\mbox{\boldmath $z$}}
\newcommand{\bg}{\mbox{\boldmath $g$}}
\newcommand{\bn}{\mbox{\boldmath $n$}}
\newcommand{\bbm}{\mbox{\boldmath $m$}}
\newcommand{\bv}{\mbox{\boldmath $v$}}
\newcommand{\bd}{\mbox{\boldmath $d$}}
\newcommand{\bQ}{\mbox{\boldmath $Q$}}
\newcommand{\bO}{\mbox{\boldmath $O$}}
\newcommand{\bR}{\mbox{\boldmath $R$}}
\newcommand{\bF}{\mbox{\boldmath $F$}}
\newcommand{\bphi}{{\bf \Phi}}
\newcommand{\bI}{\mbox{\boldmath $I$}}
\newcommand{\bbtheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bSigma}{{\bf \Sigma}}
\newcommand{\bt}{\mbox{\boldmath $t$}}
\newcommand{\bD}{\mbox{\boldmath $D$}}
\newcommand{\by}{\mbox{\boldmath $y$}}
\newcommand{\ds}{\displaystyle}
\newcommand{\bw}{\mbox{\boldmath $w$}}
\newcommand{\bY}{\mbox{\boldmath $Y$}}
\newcommand{\K}{{\cal K}}
\newcommand{\G}{{\cal G}}
\newcommand{\N}{{\cal N}_0}
\hyphenation{E-let-tro-ni-ca}
\newcommand{\bbeta}{\mbox{\boldmath{$\beta$}}}
\def\M{{\cal M}}
\def\R{{\cal R}}
\def\S{{\cal S}}
\def\I{{\cal I}}
\newcommand{\beq}{\begin{equation}}

% Set of real, integer, etc., numbers, l_2 spaces, real, and imaginary parts
\newcommand{\Reals}    {{\mathbb R}} % {{{\mathrm I\!R}}}  
\newcommand{\Cplx}      {{{\mathsf I}\!\!\!{\mathrm C}}} %{{\mathbb C}}
\newcommand{\NCplx}     {{{\mathcal{CN}}}} % Complex normal distribution
\newcommand{\Ints}      {{{\mathbb Z}}} % Z set of all integers
\newcommand{\Rats}      {{{\mathsf I}\!\!\!{\mathrm Q}}}    % Q set of all rational numbers
\newcommand{\Nats}      {{{\mathrm{ I\!N}}}} % N set of all natural numbers
\newcommand{\Tee}{      {{\mathbb T}}}
\newcommand{\ltwo}      {{\ell_2}}
\newcommand{\lone}      {{\ell_1}}
\newcommand{\Ltwo}      {{\mathbb L}^2}
\newcommand{\LtR}       {\Ltwo(\Reals)}
\newcommand{\Real}[1]   {{\mathrm{Re}\left\{#1\right\}}}
\newcommand{\Imag}[1]   {{\mathrm{Im}\left\{#1\right\}}}
\newcommand{\real}      {{\mathcal{R}} e}
\newcommand{\imag}      {{\mathcal{I}} m}



% Some commands for nice typesetting
\newcommand{\ie}        {i.~e., \hspace{2pt}}      % id est
\newcommand{\eg}        {e.~g., \hspace{2pt}}      %
\newcommand{\define}    {\stackrel{\triangle}{=}}  % define, an '=' with an '^' on top
\newcommand{\D}  {^{\dag}}               % Dagger, includes '^' !
\newcommand{\T}  {{\mathsf{T}}}          % Transpose, no '^' !
\newcommand{\ct} {{\mathsf{*}}}          % conjugate complex, should use \dag for conjugate complex transpose
\newcommand{\half}{{{^1\!\!\scriptscriptstyle{/}\!}_2}}       % a nice 1/2
\newcommand{\mrsss}[1]   {{\mathrm{\scriptscriptstyle{#1}}}}  % math roman scriptscriptstyle - works well for sub and superscripts
\newcommand{\sth}     {{\mathrm{th}}}    % superscript th \th is already defined -- the $k^\sth$ user
\newcommand{\diag}    {{\mathrm{diag}}}  % for diag{1, 2, 3}
\newcommand{\tr}      {{\mathrm{tr}}}    % trace of a matrix
\newcommand{\Res}     {{\mathrm{Res}}}   % Residue
\newcommand{\ld}      {{\mathrm{ld}}}    % logarithmus dualis
\newcommand{\barg}    {\overline{\gamma}}     % average received SNR
\newcommand{\sqgb}    {\sqrt{\barg}}     % square root of the average received SNR
\newcommand{\e}       {{\mathrm e}}      % e for exponential function
\newcommand{\E}       {{\mathrm E}}      % Expectation
\newcommand{\lNZ}     {{\lambda_{\mathsf{NZ}}}} % to denote the non-zero eigenvalues of a matrix
\newcommand{\Mt}      {{M_{\!\mrsss{T}}}}% N_T no of transmit antennas
\newcommand{\Mr}      {{M_{\!\mrsss{R}}}}% N_R no of receive antennas
\newcommand{\uple}    {{\mathrm{ul}}}    % upper-left
\newcommand{\upri}    {{\mathrm{ur}}}    % upper-right
\newcommand{\lole}    {{\mathrm{ll}}}    % lower-left
\newcommand{\lori}    {{\mathrm{lr}}}    % lower-right

% Bold numbers
\newcommand{\Zrb}     {{\mathbf 0}}      % bold zero
\newcommand{\Oneb}    {{\mathbf 1}}      % bold one

% Define bold roman letters
\newcommand{\ab}{{\mathbf a}}  \newcommand{\Ab}{{\mathbf A}}
\newcommand{\cb}{{\mathbf c}}  \newcommand{\Cb}{{\mathbf C}}
\newcommand{\db}{{\mathbf d}}  \newcommand{\Db}{{\mathbf D}}
\newcommand{\eb}{{\mathbf e}}  \newcommand{\Eb}{{\mathbf E}}
\newcommand{\fb}{{\mathbf f}}  \newcommand{\Fb}{{\mathbf F}}
\newcommand{\gb}{{\mathbf g}}  \newcommand{\Gb}{{\mathbf G}}
\newcommand{\hb}{{\mathbf h}}  \newcommand{\Hb}{{\mathbf H}}
\newcommand{\ib}{{\mathbf i}}  \newcommand{\Ib}{{\mathbf I}}
\newcommand{\jb}{{\mathbf j}}  \newcommand{\Jb}{{\mathbf J}}
\newcommand{\kb}{{\mathbf k}}  \newcommand{\Kb}{{\mathbf K}}
\newcommand{\lb}{{\mathbf l}}  \newcommand{\Lb}{{\mathbf L}}
\newcommand{\mb}{{\mathbf m}}  \newcommand{\Mb}{{\mathbf M}}
\newcommand{\nb}{{\mathbf n}}  \newcommand{\Nb}{{\mathbf N}}
\newcommand{\ob}{{\mathbf o}}  \newcommand{\Ob}{{\mathbf O}}
\newcommand{\pb}{{\mathbf p}}  \newcommand{\Pb}{{\mathbf P}}
\newcommand{\qb}{{\mathbf q}}  \newcommand{\Qb}{{\mathbf Q}}
\newcommand{\rb}{{\mathbf r}}  \newcommand{\Rb}{{\mathbf R}}
\renewcommand{\sb}{{\mathbf s}}\newcommand{\Sb}{{\mathbf S}} %\sb is equiv. to _ in Tex, unnecessary.
\newcommand{\tb}{{\mathbf t}}  \newcommand{\Tb}{{\mathbf T}}
\newcommand{\ub}{{\mathbf u}}  \newcommand{\Ub}{{\mathbf U}}
\newcommand{\vb}{{\mathbf v}}  \newcommand{\Vb}{{\mathbf V}}
\newcommand{\wb}{{\mathbf w}}  \newcommand{\Wb}{{\mathbf W}}
\newcommand{\xb}{{\mathbf x}}  \newcommand{\Xb}{{\mathbf X}}
\newcommand{\yb}{{\mathbf y}}  \newcommand{\Yb}{{\mathbf Y}}
\newcommand{\zb}{{\mathbf z}}  \newcommand{\Zb}{{\mathbf Z}}

% Define bold greek letters, lower and upper case
\newcommand{\alphab}      {{\bm \alpha}}          \newcommand{\Alphab}   {{\mathbf {\mathrm A}}}
\newcommand{\betab}       {{\bm \beta}}           \newcommand{\Betab}    {{\mathbf {\mathrm B}}}
\newcommand{\gammab}      {{\bm \gamma}}          \newcommand{\Gammab}   {{\bm \Gamma}}
\newcommand{\deltab}      {{\bm \delta}}          \newcommand{\Deltab}   {{\bm \Delta}}
\newcommand{\epsilonb}    {{\bm \epsilon}}        \newcommand{\Epsilonb} {{\mathbf {\mathrm E}}}
\newcommand{\varepsilonb} {{\bm \varepsilon}}
\newcommand{\vepsilonb}   {{\bm \varepsilon}}
\newcommand{\zetab}       {{\bm \zeta}}           \newcommand{\Zetab}    {{\mathbf {\mathrm Z}}}
\newcommand{\etab}        {{\bm \eta}}            \newcommand{\Etab}     {{\mathbf {\mathrm H}}}
\newcommand{\thetab}      {{\bm \theta}}          \newcommand{\Thetab}   {{\bm \Theta}}
\newcommand{\varthetab}   {{\bm \vartheta}}
\newcommand{\vthetab}     {{\bm \vartheta}}
\newcommand{\iotab}       {{\bm \iota}}           \newcommand{\Iotab}    {{\mathbf {\mathrm I}}}
\newcommand{\kappab}      {{\bm \kappa}}          \newcommand{\Kappab}   {{\mathbf {\mathrm K}}}
\newcommand{\lambdab}     {{\bm \lambda}}         \newcommand{\Lambdab}  {{\bm \Lambda}}
\newcommand{\mub}         {{\bm \mu}}             \newcommand{\Mub}      {{\mathbf {\mathrm M}}}
\newcommand{\nub}         {{\bm \nu}}             \newcommand{\Nub}     	{{\mathbf {\mathrm N}}}	
\newcommand{\xib}         {{\bm \xi}}             \newcommand{\Xib}      {{\bm \Xi}}
\newcommand{\omicronb}    {{\mathbf {\mathrm o}}} \newcommand{\Omicronb} {{\mathbf {\mathrm O}}}
\newcommand{\pib}         {{\bm \pi}}             \newcommand{\Pib}      {{\bm \Pi}}
\newcommand{\varpib}      {{\bm \varpi}}
\newcommand{\vpib}        {{\bm \varpi}}
\newcommand{\rhob}        {{\bm \rho}}            \newcommand{\Rhob}     {{\mathbf {\mathrm P}}}
\newcommand{\varrhob}     {{\bm \varrho}}
\newcommand{\vrhob}       {{\bm \varrho}}
\newcommand{\sigmab}      {{\bm \sigma}}          \newcommand{\Sigmab}   {{\bm \Sigma}}
\newcommand{\varsigmab}   {{\bm \varsigma}}
\newcommand{\vsigmab}     {{\bm \varsigma}}
\newcommand{\taub}        {{\bm \tau}}            \newcommand{\Taub}     {{\mathbf {\mathrm T}}}
\newcommand{\upsilonb}    {{\bm \upsilon}}        \newcommand{\Upsilonb} {{\bm \Upsilon}}
\newcommand{\phib}        {{\bm \phi}}            \newcommand{\Phib}     {{\bm \Phi}}
\newcommand{\varphib}     {{\bm \varphi}}
\newcommand{\vphib}       {{\bm \varphi}}
\newcommand{\chib}        {{\bm \chi}}            \newcommand{\Chib}     {{\mathbf {\mathrm X}}}
\newcommand{\psib}        {{\bm \psi}}            \newcommand{\Psib}     {{\bm \Psi}}
\newcommand{\omegab}      {{\bm \omega}}          \newcommand{\Omegab}   {{\bm \Omega}}

% Calligraphic letters, normal and bold
\newcommand{\Ac} {{\mathcal A}}         \newcommand{\Ak} {{\bm {\mathcal A}}}
\newcommand{\Bc} {{\mathcal B}}         \newcommand{\Bk} {{\bm {\mathcal B}}}
\newcommand{\Cc} {{\mathcal C}}         \newcommand{\Ck} {{\bm {\mathcal C}}}
\newcommand{\Dc} {{\mathcal D}}         \newcommand{\Dk} {{\bm {\mathcal D}}}
\newcommand{\Ec} {{\mathcal E}}         \newcommand{\Ek} {{\bm {\mathcal E}}}
\newcommand{\Fc} {{\mathcal F}}         \newcommand{\Fk} {{\bm {\mathcal F}}}
\newcommand{\Gc} {{\mathcal G}}         \newcommand{\Gk} {{\bm {\mathcal G}}}
\newcommand{\Hc} {{\mathcal H}}         \newcommand{\Hk} {{\bm {\mathcal H}}}
\newcommand{\Ic} {{\mathcal I}}         \newcommand{\Ik} {{\bm {\mathcal I}}}
\newcommand{\Jc} {{\mathcal J}}         \newcommand{\Jk} {{\bm {\mathcal J}}}
\newcommand{\Kc} {{\mathcal K}}         \newcommand{\Kk} {{\bm {\mathcal K}}}
\newcommand{\Lc} {{\mathcal L}}         \newcommand{\Lk} {{\bm {\mathcal L}}}
\newcommand{\Mc} {{\mathcal M}}         \newcommand{\Mk} {{\bm {\mathcal M}}}
\newcommand{\Nc} {{\mathcal N}}         \newcommand{\Nk} {{\bm {\mathcal N}}}
\newcommand{\Oc} {{\mathcal O}}         \newcommand{\Ok} {{\bm {\mathcal O}}}
\newcommand{\Pc} {{\mathcal P}}         \newcommand{\Pk} {{\bm {\mathcal P}}}
\newcommand{\Qc} {{\mathcal Q}}         \newcommand{\Qk} {{\bm {\mathcal Q}}}
\newcommand{\Rc} {{\mathcal R}}         \newcommand{\Rk} {{\bm {\mathcal R}}}
\newcommand{\Sc} {{\mathcal S}}         \newcommand{\Sk} {{\bm {\mathcal S}}}
\newcommand{\Tc} {{\mathcal T}}         \newcommand{\Tk} {{\bm {\mathcal T}}}
\newcommand{\Uc} {{\mathcal U}}         \newcommand{\Uk} {{\bm {\mathcal U}}}
\newcommand{\Vc} {{\mathcal V}}         \newcommand{\Vk} {{\bm {\mathcal V}}}
\newcommand{\Wc} {{\mathcal W}}         \newcommand{\Wk} {{\bm {\mathcal W}}}
\newcommand{\Xc} {{\mathcal X}}         \newcommand{\Xk} {{\bm {\mathcal X}}}
\newcommand{\Yc} {{\mathcal Y}}         \newcommand{\Yk} {{\bm {\mathcal Y}}}
\newcommand{\Zc} {{\mathcal Z}}         \newcommand{\Zk} {{\bm {\mathcal Z}}}


\newcommand{\Grb}   {{\mathbf {\mathrm V}}}

\newcommand{\Qulk} {{\underline{{\bm {\mathcal Q}}}}}

\newcommand{\Gulc} {{\underline{\mathcal G}}}
\newcommand{\Culc} {{\underline{\mathcal C}}}

% underlined upper and lower case letters
\newcommand{\Aul}  {{\underline A}}              \newcommand{\aul}  {{\underline a}}
\newcommand{\Bul}  {{\underline B}}              \newcommand{\bul}  {{\underline b}}
\newcommand{\Cul}  {{\underline C}}              \newcommand{\cul}  {{\underline c}}
\newcommand{\Dul}  {{\underline D}}              \newcommand{\dul}  {{\underline d}}
\newcommand{\Eul}  {{\underline E}}              \newcommand{\eul}  {{\underline e}}
\newcommand{\Ful}  {{\underline F}}              \newcommand{\ful}  {{\underline f}}
\newcommand{\Gul}  {{\underline G}}              \newcommand{\gul}  {{\underline g}}
\newcommand{\Hul}  {{\underline H}}              \newcommand{\hul}  {{\underline h}}
\newcommand{\Iul}  {{\underline I}}              \newcommand{\iul}  {{\underline i}}
\newcommand{\Jul}  {{\underline J}}              \newcommand{\jul}  {{\underline j}}
\newcommand{\Kul}  {{\underline K}}              \newcommand{\kul}  {{\underline k}}
\newcommand{\Lul}  {{\underline L}}              \newcommand{\lul}  {{\underline l}}
\newcommand{\Mul}  {{\underline M}}              \newcommand{\mull} {{\underline m}}
\newcommand{\Nul}  {{\underline N}}              \newcommand{\nul}  {{\underline n}}
\newcommand{\Oul}  {{\underline 0}}              \newcommand{\oul}  {{\underline o}}
\newcommand{\Pul}  {{\underline P}}              \newcommand{\pul}  {{\underline p}}
\newcommand{\Qul}  {{\underline Q}}              \newcommand{\qul}  {{\underline q}}
\newcommand{\Rul}  {{\underline R}}              \newcommand{\rul}  {{\underline r}}
\newcommand{\Sul}  {{\underline S}}              \newcommand{\sul}  {{\underline s}}
\newcommand{\Tul}  {{\underline T}}              \newcommand{\tul}  {{\underline t}}
\newcommand{\Uul}  {{\underline U}}              \newcommand{\uul}  {{\underline u}}
\newcommand{\Vul}  {{\underline V}}              \newcommand{\vul}  {{\underline v}}
\newcommand{\Wul}  {{\underline W}}              \newcommand{\wul}  {{\underline w}}
\newcommand{\Xul}  {{\underline X}}              \newcommand{\xul}  {{\underline x}}
\newcommand{\Yul}  {{\underline Y}}              \newcommand{\yul}  {{\underline y}}
\newcommand{\Zul}  {{\underline Z}}              \newcommand{\zul}  {{\underline z}}

% Misc. short-cuts
\newcommand{\mc}[1]     {{\mathcal{#1}}}        % mathcal
\newcommand{\what}[1]   {\widehat{#1}}          % widehat
\newcommand{\wtld}[1]   {\widetilde{#1}}        % widetilde
\newcommand{\Portho}[1] {\Pb_{#1}^{\perp}}      % orthogonal projection

%\newcounter{MYtempeqncnt}
%\setlength\arraycolsep{2pt} \sloppy

%\newcommand{\threshold}{\mbox{$
%\begin{array}{c} \stackrel{\textstyle H_1}{\textstyle>}\\
%\stackrel{\textstyle <}{\textstyle H_0}
%\end{array}$}}
%\newcommand{\nchoosek}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
%\newcommand{\gammabar}{\bar{\gamma}}
%\newcommand{\Prob}{\mbox{Prob}}

%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\setlength\arraycolsep{2pt} \sloppy

\newtheorem{definition}{Definition}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
%\newtheorem{algorithm}{Algorithm}
%\newtheorem{proof}{Proof}

\def\IR{{\mathbb R}}
\def\IC{{\mathbb C}}

